A Note on the Permuted Puzzles Toy Conjecture

In this note, we show that a "Toy Conjecture" made by (Boyle, Ishai, Pass, Wootters, 2017) is false, and propose a new one. Our attack does not falsify the full ("non-toy") conjecture in that work, and it is our hope that this note will help further the analysis of that conjecture. Independently, (Boyle, Holmgren, Ma, Weiss, 2021) have obtained similar results.

==> mary_macros.tex <==
% some packages

\usepackage[margin=1.125in]{geometry}
\usepackage{xcolor}
\definecolor{DarkGreen}{rgb}{0.1,0.5,0.1}
\definecolor{DarkRed}{rgb}{0.5,0.1,0.1}
\definecolor{DarkBlue}{rgb}{0.1,0.1,0.5}

\usepackage[small]{caption}
\usepackage[pdftex]{hyperref}
\hypersetup{
    unicode=false,          % non-Latin characters in Acrobat¿s bookmarks
    pdftoolbar=true,        % show Acrobat toolbar?
    pdfmenubar=true,        % show Acrobat menu?
    pdffitwindow=false,      % page fit to window when opened
    pdfnewwindow=true,      % links in new window
    colorlinks=true,       % false: boxed links; true: colored links
    linkcolor=DarkBlue,          % color of internal links
    citecolor=DarkGreen,        % color of links to bibliography
    filecolor=DarkGreen,      % color of file links
    urlcolor=DarkBlue,          % color of external links
    %
    % paper specific, please udpate
    %
    pdftitle={},
    pdfauthor={},    
    %pdfsubject={},
    %pdfkeywords={keywords}, % list of keywords
}
%\usepackage{hyperref,cite}
\usepackage{amssymb,amsmath,amsthm,amsfonts,enumitem}
\usepackage{fullpage,nicefrac,comment}
\usepackage{tikz}
\usetikzlibrary{arrows,decorations.pathmorphing,decorations.shapes,snakes,patterns,positioning}
\usepackage[ruled,linesnumbered]{algorithm2e}

\newcommand{\bits}{\left\{0,1\right\}}

%% common special letters
\newcommand{\A}{\ensuremath{\mathcal{A}}}
\newcommand{\B}{\ensuremath{\mathcal{B}}}
\newcommand{\I}{\ensuremath{\mathcal{I}}}
\newcommand{\cC}{\ensuremath{\mathcal{C}}}
\newcommand{\cU}{\ensuremath{\mathcal{U}}}
\newcommand{\cD}{\ensuremath{\mathcal{D}}}
\newcommand{\N}{\ensuremath{\mathcal{N}}}
\renewcommand{\L}{\ensuremath{\mathcal{L}}}
\newcommand{\R}{{\mathbb R}}
\newcommand{\Z}{{\mathbb Z}}
\newcommand{\ZZ}{{\mathbb Z}}
\newcommand{\F}{{\mathbb F}}
\newcommand{\Q}{{\mathbb Q}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}
%\newcommand{\C}{{\mathbb C}}

%% probability 
\newcommand{\PR}[1]{{\mathbb{P}}\left\{ #1\right\}}
\newcommand{\E}[1]{\mathbb{E}\left[ #1\right]}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\Eover}[2]{\mathbb{E}_{#1}\left[ #2 \right]}
\newcommand{\Var}[1]{\mathrm{Var}\left( #1\right)}
\newcommand{\pmoment}[2]{\inparen{ \EE \left| #1 \right|^#2 }^{1/#2}}

%% norms 
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\twonorm}[1]{\left\|#1\right\|_2}
\newcommand{\onenorm}[1]{\left\|#1\right\|_1}
\newcommand{\infnorm}[1]{\left\|#1\right\|_\infty}
\newcommand{\opnorm}[1]{\left\|#1\right\|}
\newcommand{\nucnorm}[1]{\left\|#1\right\|_*}
\newcommand{\decnorm}[2]{\left\|#1\right\|_{#2}}
\newcommand{\fronorm}[1]{\decnorm{#1}{F}}
\newcommand{\gaunorm}[1]{\decnorm{#1}{\psi_2}}
\newcommand{\expnorm}[1]{\decnorm{#1}{\psi_1}}
\newcommand{\orliczp}[2]{\decnorm{#1}{\psi_{#2}}}
\newcommand{\inabs}[1]{\left|#1\right|}
%% inner products
\newcommand{\ip}[2]{\ensuremath{\left\langle #1,#2\right\rangle}}
\newcommand{\ket}[1]{\left|#1\right\rangle}
\newcommand{\bra}[1]{\left\langle#1\right|}
\newcommand{\braket}[2]{\left\langle #1 \right|\left. #2 \right\rangle}
%% (), {}, etc
\newcommand{\inset}[1]{\left\{#1\right\}}
\newcommand{\inbrac}[1]{\left\{#1\right\}}
\newcommand{\inparen}[1]{\left(#1\right)}
\newcommand{\inbrak}[1]{\left[#1\right]}
\newcommand{\suchthat}{\,:\,}
\newcommand{\rg}[2]{\{#1,\ldots,#2\}}

%% products
\newcommand{\had}{\circ}
\newcommand{\tensor}{\otimes}

%% useful words
\newcommand{\supp}{\mathrm{Supp}}
\newcommand{\agr}{\mathrm{agr}}
\newcommand{\conv}{\operatorname{conv}}
\newcommand{\argmax}{\mathrm{argmax}}
\newcommand{\argmin}{\mathrm{argmin}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\median}{\ensuremath{\operatorname{median}}}
\newcommand{\Vol}{\ensuremath{\operatorname{Vol}}}
\newcommand{\rank}{\ensuremath{\operatorname{rank}}}
\newcommand{\spn}{\ensuremath{\operatorname{span}}}
\newcommand{\dist}{\ensuremath{\operatorname{dist}}}
\newcommand{\diag}{\ensuremath{\operatorname{diag}}}
\newcommand{\diam}{\ensuremath{\operatorname{diam}}}
\newcommand{\tr}{\mathrm{tr}}
\newcommand{\sgn}{\mathrm{sign}}
\newcommand{\Hom}{\ensuremath{\operatorname{Hom}}}
\newcommand{\Ker}{\ensuremath{\operatorname{Ker}}}
\newcommand{\Ann}{\ensuremath{\operatorname{Ann}}}

%%% misc
\newcommand{\frakp}{\ensuremath{\mathfrak{p}}}
\newcommand{\frakq}{\ensuremath{\mathfrak{q}}}
\newcommand{\intring}{{\mathcal O}}

\newcommand{\divides}{\mbox{ {\Large $|$} } }
\newcommand{\bigoh}{\mathcal{O}}
\newcommand{\hf}{\frac{1}{2}}
\newcommand{\nicehf}{\ensuremath{\nicefrac{1}{2}}}

\newcommand{\dd}[2]{\frac{\partial #1}{\partial #2} }
\newcommand{\ind}[1]{\ensuremath{\mathbf{1}_{#1}}}
\newcommand{\n}{\newline}

\newcommand{\anaught}{\aleph_0}
\newcommand{\contin}{2^{\aleph_0}}
\newcommand{\preomega}{{}^\omega}

\renewcommand{\sp}[1]{^{(#1)}}

%% OMG curly greek letters
\newcommand{\eps}{\varepsilon}
\renewcommand{\epsilon}{\varepsilon}
\newcommand{\vphi}{\varphi}
\newcommand{\vpsi}{\varpsi}

%% comments
\newcommand{\mkw}[1]{{\footnotesize  [\textbf{\textcolor{blue}{#1}} \textcolor{blue!60!black}{--mary}]\normalsize}}
\newcommand{\TODO}[1]{\textcolor{red}{\textbf{TODO: #1}}}
\newcommand{\BIGTODO}[1]{\Large\textcolor{red}{\textbf{TODO: #1}}\normalsize}

%% thm environments
\newtheorem{theorem}{Theorem} 
\newtheorem{lemma}[theorem]{Lemma} 
\newtheorem{definition}{Definition} 
\newtheorem{protodefinition}[theorem]{proto-Definition} 
\newtheorem{obs}[theorem]{Observation} 
\newtheorem{observation}[theorem]{Observation} 
\newtheorem{conjecture}[theorem]{Conjecture} 
\newtheorem{cor}[theorem]{Corollary} 
\newtheorem{corollary}[theorem]{Corollary} 
\newtheorem{stupid}[theorem]{Stupid Theorem}
\newtheorem{remark}{Remark}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{prop}[theorem]{Proposition}
\newtheorem{sublemma}[theorem]{Sublemma}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{want}[theorem]{Want}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{question}[theorem]{Question}
\newtheorem{example}{Example}
\newtheorem{property}{Property}

